Graph properties in node-query setting: effect of breaking symmetry

The query complexity of graph properties is well-studied when queries are on edges. We investigate the same when queries are on nodes. In this setting a graph $G = (V, E)$ on $n$ vertices and a property $\mathcal{P}$ are given. A black-box access to an unknown subset $S \subseteq V$ is provided via queries of the form `Does $i \in S$?'. We are interested in the minimum number of queries needed in worst case in order to determine whether $G[S]$, the subgraph of $G$ induced on $S$, satisfies $\mathcal{P}$. Apart from being combinatorially rich, this setting allows us to initiate a systematic study of breaking symmetry in the context of query complexity of graph properties. In particular, we focus on hereditary graph properties. The monotone functions in the node-query setting translate precisely to the hereditary graph properties. The famous Evasiveness Conjecture asserts that even with a minimal symmetry assumption on $G$, namely that of vertex-transitivity, the query complexity for any hereditary graph property in our setting is the worst possible, i.e., $n$. We show that in the absence of any symmetry on $G$ it can fall as low as $O(n^{1/(d + 1) })$ where $d$ denotes the minimum possible degree of a minimal forbidden sub-graph for $\mathcal{P}$. In particular, every hereditary property benefits at least quadratically. The main question left open is: can it go exponentially low for some hereditary property? We show that the answer is no for any hereditary property with {finitely many} forbidden subgraphs by exhibiting a bound of $\Omega(n^{1/k})$ for some constant $k$ depending only on the property. For general ones we rule out the possibility of the query complexity falling down to constant by showing $\Omega(\log n/ \log \log n)$ bound. Interestingly, our lower bound proofs rely on the famous Sunflower Lemma due to Erd\"os and Rado.

==> hereditary/temp-upper.tex <==
\section{A general upper bound}
\label{sec:upper}
Let $\mathcal{P}$ be a hereditary graph property
and $d_\mathcal{P}$ denote the minimum possible degree
of a minimal forbidden subgraph for $\mathcal{P}$.

\begin{theorem}
For any  hereditary graph property $\mathcal{P}$: \[min\text{-}cost(\mathcal{P}) = O(n^{1/(d_\mathcal{P} + 1)}).\] \label{thm:upper-d}
\end{theorem}
\begin{proof}
Let $k = \Theta(n^{1/(d_\mathcal{P}+1)})$ with an appropriately chosen constant.
Construct a graph $G$ on $n$ vertices as follows (See Figure~\ref{fig:general-upper}):
\begin{itemize}
\item start with a clique on vertices $v_1, \ldots, v_k$ 
\item for every $S \subseteq [k]$ such that $|S| = d_\mathcal{P}$
 \begin{itemize}
\item add $k$ new vertices $u_1^S, \ldots, u_k^S$ 
\item connect each $u_i^S$ to every $v_i : i \in S$.
\end{itemize}
\end{itemize}

Note that every vertex of $G$ is relevant for $\mathcal{P}$. Now we describe an algorithm to  determine $\mathcal{P}$ in $O(n^{1/(d_\mathcal{P} +1)})$ queries.
Let $c_\mathcal{P}$ denote the smallest integer such that the clique on $c_\mathcal{P}$ vertices does not satisfy $\mathcal{P}$.


\subsection*{Algorithm}
\begin{itemize}
\item query $v_1, \ldots, v_k$
\item if at least $c_\mathcal{P}$ of these vertices are present then $\mathcal{P}$ must fail.
\item otherwise there are at most $c_\mathcal{P}$ vertices present (wlog: $v_1, \ldots, v_{c_\mathcal{P}}$)
\begin{itemize}
\item for every subset $S \subseteq [c_\mathcal{P}]$ such that $|S| = d_\mathcal{P}$, query $u_1^S, \ldots, u_k^S$.
\item if the graph induced on the nodes present (after all these ${c_\mathcal{P} \choose d_\mathcal{P}} \times k$ queries) satisfies $\mathcal{P}$ then answer Yes otherwise answer No.
\end{itemize}
\end{itemize}

\subsection*{Correctness and Complexity}
Note that any vertex that is not queried by the above algorithm can have at most $d_\mathcal{P} - 1$ edges to the vertices in the clique $v_1, \ldots, v_k$.
Since $d_\mathcal{P}$ is the minimum degree of a minimal forbidden subgraph for $\mathcal{P}$, these vertices now become irrelevant for $\mathcal{P}$.
Thus the algorithm can correctly declare the answer based on only the queries it has made.
It is easy to check that the query complexity of the above algorithm is $O(k)$ which is $O(n^{1/(d_\mathcal{P}+1)})$.

\end{proof}

==> infinite-upper.tex <==
\section{Upper bounds for some infinite hereditary properties}\label{sec:infinite-upper-bound}


\begin{lemma}\label{infinite-forbidden-acyclicity}
Let $G$ be a graph on $n$ vertices, and let $\mathcal{C}$ denote the property of being acyclic. Then:

\[min\text{-}cost(\mathcal{C}) = O(n^{1/3}).\] 
\end{lemma}
 \begin{proof}
\red{Proof of this lemma would appear in the final version.}
 \end{proof} 
 
 
 \begin{lemma}\label{infinite-forbidden-bipartiteness}
Let $G$ be a graph on $n$ vertices, and let $\mathcal{B}$ denote the property of being bipartite. Then:

\[min\text{-}cost(\mathcal{B}) = O(n^{1/3}).\] 
\end{lemma}
 \begin{proof}
\red{Proof of this lemma would appear in the final version.}
 \end{proof} 
 
 \begin{lemma}\label{infinite-forbidden-planarity}
Let $G$ be a graph on $n$ vertices, and let $\mathcal{P}$ denote the property of being planar. Then:

\[min\text{-}cost(\mathcal{P}) = O(n^{1/4}).\] 
\end{lemma}
 \begin{proof}
\red{Proof of this lemma would appear in the final version.}
 \end{proof} 
 
 
  \begin{lemma}\label{infinite-forbidden-3color}
Let $G$ be a graph on $n$ vertices, and let $\mathcal{P}$ denote the property of being $3$-colorable. Then:

\[min\text{-}cost(\mathcal{C}) = O(n^{1/4}).\] 
\end{lemma}
 \begin{proof}
\red{Proof of this lemma would appear in the final version.}
 \end{proof} 
 

==> table-restriction.tex <==





\begin{comment}

\begin{table}[h]\label{table:global-vs-local}
\resizebox{\textwidth}{!}{% Scale down your table to the textwidth
\begin{tabular}{|c c|c|c|}
\hline 
\multicolumn{2}{|c|}{Properties} & With Symmetry & Without Symmetry \\
 \hline 
\hline
Connectedness & [Sec. \ref{connectivity}]  & $\Theta(n)$  & $\Theta(n)$\\
\hline
$s$-$t$ connectivity  & [Sec. \ref{connectivity}]   &  & $\Theta(\sqrt n)$\\
 \hline
Perfect Matching\footnote{out of context}  &  [Sec. \ref{perfect-matching}]  & $\Theta(n)$ &  $\Theta(n)$ \\
\hline
\end{tabular}
} %%%%%%%%%%%%%%%%%%%% closing bracket of \resizebox{\textwidth}{!}{%
\caption{Global vs. Local Phenomenon}
\end{table}
\end{comment}







\begin{table}[h]\label{table:restrictions}
\resizebox{\textwidth}{!}{%   Scale down your table to the textwidth
\begin{tabular}{|c|c c|c|c|}
\hline 
 & \multicolumn{2}{|c|}{Properties} & With Symmetry\footnote{Assuming Evasiveness Conjecture} & Without Symmetry \\
 \hline 
 \hline
\multirow{4}{*}{\begin{turn}{90}Planar\end{turn}} & Emptiness & [\ref{planar-emptiness}] & $n$ & $n/4$\\
\cline{2-5}
& Bounded Degree & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Triangle Freeness & [\ref{cor-pla-tri}] & $n$ &  $\Omega(\sqrt n)$  \\
\cline{2-5}
& Acyclicity & [\ref{planar-acyclicity}] & $n$ &   $\Omega(n^{1/100})$  \\
 \hline 
 \hline
\multirow{4}{*}{\begin{turn}{90}Outer\end{turn} \begin{turn}{90}Planar\end{turn}} & Emptiness & [\ref{outer-planar-emptiness}] & $n$ & $n/3$\\
\cline{2-5}
& Bounded Degree & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Triangle Freeness & [\ref{cor-pla-tri}] & $n$ &   $\Omega(\sqrt{n})$  \\
\cline{2-5}
& Acyclicity & [\ref{outer-planar-acyclicity}] & $n$ &  $\Omega(n^{1/100})$    \\
 \hline 
 \hline
\multirow{4}{*}{\begin{turn}{90}Bounded\end{turn} \begin{turn}{90}Degree\end{turn}} & Emptiness & [\ref{apx}] & $n$ & $n/2 +1$\\
\cline{2-5}
& Bounded Degree & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Triangle freeness & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Acyclicity & [\ref{apx}] & $n$ &     \\
\hline
 \hline 
\multirow{4}{*}{\begin{turn}{90}Bipartite\end{turn}} & Emptiness & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Bounded Degree & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Triangle Freeness & [\ref{apx}] & $n$ &     \\
\cline{2-5}
& Acyclicity & [\ref{apx}] & $n$ &     \\
\hline
\end{tabular}
} %%%%%%%%%% Closing bracket of \resizebox{\textwidth}{!}{%
\caption{Restrictions: Planar, Bounded degree, Bipartite}
\end{table}



